TxT: Real-time Transaction Encapsulation for Ethereum Smart Contracts

Ethereum is a permissionless blockchain ecosystem that supports execution of smart contracts, the key enablers of decentralized finance (DeFi) and non-fungible tokens (NFT). However, the expressiveness of Ethereum smart contracts is a double-edged sword: while it enables blockchain programmability, it also introduces security vulnerabilities, i.e., the exploitable discrepancies between expected and actual behaviors of the contract code. To address these discrepancies and increase the vulnerability coverage, we propose a new smart contract security testing approach called transaction encapsulation. The core idea lies in the local execution of transactions on a fully-synchronized yet isolated Ethereum node, which creates a preview of outcomes of transaction sequences on the current state of blockchain. This approach poses a critical technical challenge -- the well-known time-of-check/time-of-use (TOCTOU) problem, i.e., the assurance that the final transactions will exhibit the same execution paths as the encapsulated test transactions. In this work, we determine the exact conditions for guaranteed execution path replicability of the tested transactions, and implement a transaction testing tool, TxT, which reveals the actual outcomes of Ethereum transactions. To ensure the correctness of testing, TxT deterministically verifies whether a given sequence of transactions ensues an identical execution path on the current state of blockchain. We analyze over 1.3 billion Ethereum transactions and determine that 96.5% of them can be verified by TxT. We further show that TxT successfully reveals the suspicious behaviors associated with 31 out of 37 vulnerabilities (83.8% coverage) in the smart contract weakness classification (SWC) registry. In comparison, the vulnerability coverage of all the existing defense approaches combined only reaches 40.5%.

==> casestudy.tex <==

% \section{TxT Classification}
% We discover that the real world implementation of transaction encapsulation has multiple technical nuances related to propagation and admission of transactions by Ethereum nodes. To address these practical challenges, we create TxT, a user-friendly defense tool that implements the transaction encapsulation method in Ethereum. Table~\ref{table:comparison} shows the classification of TxT compared to the set of tools representing the diversity of smart contract defense approaches. We group the features describing the defense methods into 5 classes: threat model, input, core method, defense action, and targeted contracts. 
% %As we can see, each defense method can be accurately described through the perspective of these 17 binary features.
% Per this classification, \emph{TxT is a defense tool based on the transaction encapsulation method that intercepts unsafe transactions in vulnerable, malicious, and buggy Ethereum smart contracts using transaction and chain data as its input.}

% % is paved with multiple technical challenges, such as maintaining the integrity of the blockchain consensus and determining the testability of a given transaction, to name a few.
% % User interactions with crypto wallets and dApps eventually translate into blockchain transactions. 

% \begin{table}
% \setlength{\tabcolsep}{3.1pt}
%     \centering
%     \caption{Classification of TxT compared with other tools.}\label{table:comparison}
    
%     \begin{tabular}{c|c||p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}p{1mm}}    
%         \arrayrulecolor{red}\toprule
        
%         % ============ UPPER HEADERS =================
%         \multicolumn{2}{c}{} &
%         \multicolumn{14}{c}{\textit{Threat mitigation tools}} \\
%         % \cmidrule(lr){4-5} 
%         \cmidrule(lr){3-16}
    
%         % ============ LOWER HEADERS =================
%         \textbf{} &
%         \textbf{} &
%         \scriptsize \multirow[b]{6}{*}{ \rotatebox[origin=l]{90}{\hspace{-4pt} Oyente~\cite{luu2016making}}} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} Securify~\cite{tsankov2018securify} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} Mythril~\cite{mueller2018smashing} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} Sereum~\cite{rodler2018sereum} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} SODA~\cite{chen2020soda} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} SafelyAdmin.~\cite{ivanov2021rectifying} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} ZEUS~\cite{kalra2018zeus} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} ConFuzzius~\cite{ferreira2021confuzzius} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} SeRIF~\cite{cecchetti12compositional} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} SmarTest~\cite{so2021smartest} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} VerX~\cite{permenev2020verx} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} HoneyBader~\cite{torres2019art} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} TokenScope~\cite{chen2019tokenscope} }} &
%         \scriptsize \multirow[b]{6}{*}{\rotatebox[origin=l]{90}{\hspace{-4pt} \textbf{TxT (our work)}}}
%         \\
%         \textbf{} & & & & & & & & & & & & & & & \\
%         \textbf{} & & & & & & & & & & & & & & & \\
%         \textbf{} & & & & & & & & & & & & & & & \\
%         \textbf{Class} & \textbf{Feature} & & & & & & & & & & & & & & \\
%         \textbf{} & & & & & & & & & & & & & & & \\
%         \arrayrulecolor{red}\midrule
        
%         % ============ DATA =================
        
%       \multirow{3}{*}{\shortstack[l]{Threat\\Model}} & \gc Victim s.c. & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} &
%         \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51}
%         \\
        
%         & Malicious s.c. & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51}
%         \\
                
%         & \gc No adversary & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} &
%         \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} & \gc \ding{51} & \gc \ding{51}
%         \\
        
%         \arrayrulecolor{red}\midrule
        
%         \multirow{5}{*}{\shortstack[l]{Input}} & Bytecode & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{55} &
%         \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55}
%         \\
            
%         & \gc Source code & \gc \ding{55} & \gc \ding{51} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55}
%         \\
                
%         & ABI & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} &
%         \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55}
%         \\
                
%         & \gc Transactions & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} &
%         \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51}
%         \\
                
%         & Chain data & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{55} &
%         \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51}
%         \\
        
%         \arrayrulecolor{red}\midrule
            
%         \multirow{3}{*}{\shortstack[l]{Core\\Method}} & \gc Test/execute & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51}
%         \\
        
%         & Syntax analysis & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} &
%         \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55}
%         \\
        
%          & \ggc \textbf{Encapsulation} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} &
%         \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{55} & \ggc \ding{51}
%         \\

%         \arrayrulecolor{red}\midrule
        
%         \multirow{3}{*}{\shortstack[l]{Defense\\Action}} & \gc Report & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55}
%         \\
        
%         & Code patch & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55}
%         \\
                
%         & \gc Interception & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} & \gc \ding{51} & \gc \ding{55} &
%         \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51}
%         \\
        
%         \arrayrulecolor{red}\midrule
        
%         \multirow{3}{*}{\shortstack[l]{Targeted\\Contracts}} & Any Ethereum & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51}
%         \\
                
%         & \gc Specific type$\mathrm{^\dagger}$ & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} &
%         \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{55} & \gc \ding{51} & \gc \ding{55}
%         \\
        
%         & Non-Ethereum & \ding{55} & \ding{55} & \ding{55} &  \ding{55} & \ding{51} & \ding{55} &
%         \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55}
%         \\
        
%         % ============ LEGEND: ICONS =================
%         \arrayrulecolor{red}\bottomrule
%         % \multicolumn{16}{c}{\scriptsize
%         % \CIRCLE~--- full support; \LEFTcircle~--- partial support; \Circle~--- no support; \faQuestionCircle~--- possible support (insufficient data); {\scriptsize \faWarning}~--- possibility warning.
%         % } \\
%         % \arrayrulecolor{red}\hline
%         % ============ LEGEND: SUPERSCRIPTS =================
%         \multicolumn{16}{l}{$\mathrm{^\dagger}$ e.g., ERC-20, ERC-721, etc.}
%     \end{tabular}
%     \vspace{-10pt}
% \end{table}

\section{Case Study}\label{sec:casestudy}

\subsection{Execution Sequences}
In order to comprehensibly observe the execution of a transaction sequence, we introduce a concise execution trace language $\langle \phi \rangle$ with the following grammar:
% \begin{verbatim}
% <phi> ::= <tx> | <phi> "\n" <tx>
% <tx> ::= <contract> "." <function> "(" <arguments> ")" "[" <statedesc> "]"
% <contract> ::= <terminus>
% <function> ::= <terminus>
% <arguments> ::= <assn> | <assn> "," <arguments>
% <statedesc> ::= <assn> | <assn> "," <statedesc>
% <assn> ::= <terminus> "=" <terminus>
% <terminus> ::= ([1-9] | [A-Z] | [a-z])+    
% \end{verbatim}
\[
\begin{array}{l}
\langle \phi \rangle ::= \langle T \rangle \; | \; \langle \phi \rangle \hookleftarrow \langle T \rangle \\
\langle T \rangle ::= \Psi : \Omega . \Omega \; ( \langle B \rangle ) \; [ \langle A \rangle ] \\
\;\;\;\;\;\;\;\;\;\;|\; \Psi : \Omega . \Omega \; ( \langle B \rangle ) \; \hookleftarrow \; \langle T \rangle \; \hookleftarrow \; [ \langle A \rangle ] \\
% \langle C \rangle ::= \Omega \\
% \langle F \rangle ::= \Omega \\
\langle B \rangle ::= \langle L \rangle \\
\langle A \rangle ::= \langle L \rangle \; | \; \text{REVERT} \\
\langle L \rangle ::= \varnothing \; | \; \langle M \rangle \; | \; \langle M \rangle , \langle L \rangle \\
\langle M \rangle ::= \Omega = \Omega \\
\end{array}
\]
%\commentnick{TODO: Explain the newline symbols and terminals in this syntax.}
Here, $\Omega$ is terminal text for identifiers and literals, $\Psi$ is a numerical literal for counting transactions, and $\hookleftarrow$ is the newline. $\langle T \rangle$ represents a transaction, $\langle B \rangle$ represents the list of pre-conditions (the state before execution of the transaction), $\langle A \rangle$ is a post-condition (the state after execution), $\langle L \rangle$ is a list of state assignments, and $\langle M \rangle$ is a single assignment in the form of $parameter=value$. $REVERT$ is a special statement signifying a failed transaction.
%\commentyan{what is A, B, M, L, REVERT}\commentnick{DONE}
This syntax allows to represent the execution 
%of a sequence of transactions 
in a series of terse statements by eliminating unnecessary information, such as irrelevant variables. Also, it allows to use named parameters in lieu of actual values whenever necessary. For example, a sample execution trace of a series of transactions applied to the smart contract in Fig.~\ref{fig:motivation} is as follows:
% \[
% \small
% \begin{array}{l}
% \text{\ding{182}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Foo.deposit}}}} \\
% \;\;\textbf{(}\textcolor{Color002}{\textit{msg.value}}=1\;\text{ether},
% \textcolor{Color002}{\textit{this.balance}}=0\textbf{)} \\
% \;\;\textbf{\lbrack} \textcolor{Color002}{\textit{msg.sender.balance}}=A_b - 1\;\text{ether}, \textcolor{Color002}{\textit{this.balance}}= 1\;\text{ether} \textbf{\rbrack} \\
% \text{\ding{183}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Foo.withdraw}}}} \\
% \;\;\textbf{(}\textcolor{Color002}{\textit{this.balance}}=1\;\text{ether},
% \textcolor{Color002}{\textit{msg.sender.balance}}=A_b\textbf{)} \\
% \;\;\textbf{\lbrack} \textcolor{Color002}{\textit{msg.sender.balance}}=A_b + 0.999999999\;\text{ether}, \\ \;\;\textcolor{Color002}{\textit{this.balance}}=0\;\text{ether},
% \;\;\textcolor{Color002}{\textit{admin.balance}}=1000000000\;\text{wei} \textbf{\rbrack} \\
% \end{array}
% \]
% The failed execution of the same smart contract, after redeployment on the Mainnet, may be traced as follows:
\[
\small
\begin{array}{l}
\text{\ding{182}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Foo.deposit}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.value}}=1\;\text{ether},
\textcolor{Color002}{\textit{this.balance}}=0\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textit{msg.sender.balance}}=A_b - 1\;\text{ether}, \textcolor{Color002}{\textit{this.balance}}= 1\;\text{ether} \textbf{\rbrack} \\
\text{\ding{183}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Foo.withdraw}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{this.balance}}=1\;\text{ether},
\textcolor{Color002}{\textit{msg.sender.balance}}=A_b - 1\;\text{ether}\textbf{)} \\

\;\;\;\;\text{\ding{184}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Bar.fallback}}}} \\
\;\;\;\;\;\;\textbf{(}\textcolor{Color002}{\textit{msg.value}}=1000000000\;\text{wei}\textbf{)} \\
\;\;\;\;\;\;\textbf{\lbrack} \textcolor{Color002}{\textbf{\textit{REVERT}}} \textbf{\rbrack} \\
\;\; \textbf{\lbrack} \textcolor{Color002}{\textbf{\textit{REVERT}}} \textbf{\rbrack} \\
\end{array}    
\]

In this trace, every numbered entry represents execution of a single transaction or ICC call. Each entry starts with the contract name and function name, followed by the list of selected pre-conditions in parentheses, concluded by the list of post-conditions in square brackets.


In this section, we demonstrate how TxT defends against various types of smart contract vulnerabilities. We showcase four cases divided into two groups: the real-world cases and novel (hypothetical) cases. We demonstrate that TxT is capable of defending against vulnerabilities and unpredictable behavior in different scenarios, from traditional vulnerabilities to zero-day vulnerabilities to social engineering attacks.

\subsection{Real-World Cases}\label{sec:realcases}
Here, we demonstrate how TxT detects two real-world cases that existing defense tools fail to capture.

\subsubsection{Case 1: Known Vulnerabilities}
\begin{figure}[t]
    \centering
    \lstinputlisting[language=Solidity]{listings/case1.txt}
    \vspace{-10pt}
    \caption{Case 1: A combination of SWC-132 ``Unexpected Ether'' and SWC-110 ``Assertion Violation'' vulnerabilities.}
    \label{fig:case1}
    \vspace{-10pt}
\end{figure}

Consider the smart contract in Fig.~\ref{fig:case1}, which has two vulnerabilities: ``Unexpected Ether'' (SWC-132) and ``Assertion Violation'' (SWC-110). This contract allows to make a single deposit and later withdraw the contract balance by the owner of the contract. When the smart contract is deployed, the \texttt{deposit\_made} variable is set to \texttt{false}. This variable is used by the contract to enforce the workflow in which one deposit is followed by a single withdrawal. This functionality works impeccably if the smart contract is deployed by a transaction without a value.
%However, this smart contract has a hidden SWC-132 vulnerability that may cause a financial damage to its owner.
However, if the smart contract is deployed with a positive value\footnote{Calling \emph{with value} means that the the transaction transfers some Ether to the smart contract \emph{before} executing the code of the function.} (e.g., 1 Ether), the money will be trapped in the contract forever due to the inability to make a deposit or withdraw.
% caused by the combination of the ``Unexpected Ether'' (SWC-132) vulnerability and the ``Assertion Violation'' (SWC-110) vulnerability.
The following execution trace demonstrates how this vulnerability works:
\[
\small
\begin{array}{l}
\text{\ding{182}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Foo.constructor}}}} \\
\;\; \textbf{(} \textcolor{Color002}{\textit{msg.sender}} = A_d, \textcolor{Color002}{\textit{msg.value}} = 1\;\text{ether}
\textbf{)} \\
\;\; \textbf{\lbrack} \textcolor{Color002}{\textit{owner}} = A_d, \textcolor{Color002}{\textit{deposit\_made}} = false, \textcolor{Color002}{\textit{this.balance}} = 1\;\text{ether} \textbf{\rbrack} \\

\text{\ding{183}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Foo.deposit}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.value}}=1\;\text{ether}, \textcolor{Color002}{\textit{this.balance}} = 1\;\text{ether}, \\
\;\;\textcolor{Color002}{\textit{deposit\_made}} = false
\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textbf{\textit{REVERT}}} \textbf{\rbrack} \\

\text{\ding{184}}\;\mathrm{\texttt{\textcolor{Color001}{\textbf{Foo.withdraw}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}}=A_d, \textcolor{Color002}{\textit{this.balance}} = 1\;\text{ether},\\
\;\;\textcolor{Color002}{\textit{deposit\_made}} = false
\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textbf{\textit{REVERT}}} \textbf{\rbrack}
\end{array}    
\]

TxT unambiguously reveals the unexpected behavior to the user in the case when the smart contract was deployed with a positive value, i.e., the attempt to test the deposit transaction will produce a transaction failure error displayed in the wallet.
% , the test transaction will \emph{not} show the reduced balance of the user account, neither will it show the increased balance of the smart contract as part of its a posteriori state, so the user will be able to reveal a problem after a quick look at the account balance in the wallet.

\subsubsection{Case 2: Ambiguous Semantic}

\begin{figure}[t]
    \centering
    \lstinputlisting[language=Solidity]{listings/case2.txt}
    \vspace{-10pt}
    \caption{Case 2: Smart contract with an ambiguous semantic.}
    \label{fig:case2}
    \vspace{-10pt}
\end{figure}

Consider the real-world smart contract shown in Fig.~\ref{fig:case2}\footnote{Published at \texttt{0x92B994f8F4422EaBf79d469B25958f08504160E0} on Ethereum Mainnet, with the source code shared under the MIT License.}. This contract sets up an owner by initializing the \texttt{owner} variable in the constructor. %The constructor is invoked only once during the deployment of the smart contract, and the address of the deploying account 
% (temporarily stored in \texttt{msg.sender} variable\footnote{The lifetime of \texttt{msg.sender} is limited to the current transaction.}) 
%is assigned to the permanent variable \texttt{owner}.
The \texttt{deposit()} function of the smart contract has the \texttt{payable} modifier that allows to call this function with value. This function allows the owner to deposit funds on the contract, while prohibiting any other account from doing the same. The \texttt{withdraw()} function transfers the balance of the smart contract to the caller of the function.

The eccentricity of this smart contract is in the fact that the deposit of funds is protected, while the withdrawal is not, which contradicts common sense.
The purpose of this odd behavior is unknown: it could be a honeypot, a mere bug, or an \emph{Ether faucet} --- a contract altruistically distributing funds among members of the Ethereum community.
% This contract might have been deployed for learning purposes, or this odd behavior could signify a code bug. Also, the smart contract could be a honeypot~\cite{torres2019art}. Finally, the smart contract could be an \emph{Ether faucet} --- altruistically distributing funds among members of the Ethereum community. 
%Nevertheless, the code of the contract, along with its transaction history, would be insufficient to understand the reason why this contract was deployed.

In the meantime, the \texttt{withdraw()} function exhibits a vulnerability SWC-105 (``Unprotected Ether Withdrawal''), which is detectable by some existing defense tools~\cite{brent2018vandal, tsankov2018securify}. 
%, such as Vandal~\cite{brent2018vandal} and Securify~\cite{tsankov2018securify}. 
Although TxT does not allow to defend against all SWC-105 instances, in this specific case TxT can deterministically confirm that at the moment the invocation of the \texttt{withdraw()} function of the smart contract indeed ensues the transfer of funds from the contract to the sender of the transaction, as demonstrated in the following trace:
\[
\small
\begin{array}{l}
\text{\ding{182}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Contract.constructor}}}} \; \textbf{(} \textcolor{Color002}{\textit{msg.sender}} = A_d \textbf{)}
\;\textbf{\lbrack} \textcolor{Color002}{\textit{owner}} = A_d \textbf{\rbrack} \\
\text{\ding{183}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{Contract.deposit}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.value}}=V_1, \textcolor{Color002}{\textit{msg.sender}} = A_d, \textcolor{Color002}{\textit{this.balance}} = 0\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textit{this.balance}} = V_1 \textbf{\rbrack} \\
\text{\ding{184}}\;\mathrm{\texttt{\textcolor{Color001}{\textbf{Contract.withdraw}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}}=A_d, \textcolor{Color002}{\textit{this.balance}} = V_1, \textcolor{Color002}{\textit{msg.sender.balance}} = V_2\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textit{this.balance}} = 0, \textcolor{Color002}{\textit{msg.sender.balance}} = V_1 + V_2 \textbf{\rbrack}
\end{array}    
\]

This case shows that the presence of a footprint of a vulnerability in the code does not necessarily imply that the smart contract is vulnerable or malicious. In this scenario, the traditional defense approach faces a conundrum: if the smart contract is an Ether faucet, the detection of the SWC-105 vulnerability constitutes a false positive result. This smart contract illustrates that neither the code nor the transaction history allow us to confidently argue about the safety of a smart contract. TxT approaches this case in a new way: it provides the user with a test-drive network for Ethereum transactions, removing the overwhelming burden of understanding the semantic of the smart contract. 

% Specifically, if the user is not the owner of this smart contract, the testing workflow, from the user's perspective, will be as follows:
% \begin{itemize}
%     \item[\ding{182}] The user chooses the TxT network in their wallet.
%     \item[\ding{183}] The user calls the \texttt{deposit()} function of the smart contract (directly or via a dApp).
%     \item[\ding{184}] Soon after that, the wallet shows that the transaction has been reverted.
%     \item[\ding{185}] The user sees the unexpected outcome and abandons the transaction.
% \end{itemize}

% Now, let us observe the user-side workflow of calling the \texttt{withdraw()} function, assuming the balance of the contract is 1 Ether:
% \begin{itemize}
%     \item[\ding{182}] The user chooses the TxT network in the wallet.
%     \item[\ding{183}] The user calls the \texttt{withdraw()} function of the smart contract.
%     \item[\ding{184}] Soon after that, the wallet shows that the Ether balance of the wallet increased by 1 Ether.
%     \item[\ding{185}] The user switches to Mainnet network in their wallet.
%     \item[\ding{186}] The user opens up the personal TxT transaction panel in the web browser, which shows that the last transaction (step \ding{183}) is testable and valid.
%     \item[\ding{187}] The user calls the \texttt{withdraw()} function using the Mainnet network.
% \end{itemize}

% As we can see, TxT allows to test Ethereum transactions without installing new software or scrutinizing the source code of the smart contract. This makes TxT the first user-friendly smart contract defense tool.

% Specifically, for each transaction, it is necessary to understand the expected behavior of the smart contract --- the transaction semantic. In this work, we undertake the first attempt to incorporate the transaction semantic into the security audit workflow by allowing the user to observe what exactly would have happened if a given transaction had been submitted to Ethereum Mainnet.
%\commentyan{Feel like here: we need to provide what users really observe with our tool. }\commentnick{DONE}



\subsection{Novel Cases}\label{sec:realcases}
Next, we demonstrate the workings of TxT using two interesting novel smart contract cases: a zero-day vulnerability and a social engineering attack.

\subsubsection{Case 3: Zero-day Vulnerability}
\begin{figure}[t]
    \centering
    \lstinputlisting[language=Solidity]{listings/case3.txt}
    \vspace{-10pt}
    \caption{Case 3: Zero-day ``Boolean Deadlock'' vulnerability.}
    \label{fig:case3}
    \vspace{-10pt}
\end{figure}

%As part of our another research project,
In our research, we discover some zero-day vulnerabilities, which are neither included in the SWC Registry nor mentioned (to the best of our knowledge) in any other public sources. One of these vulnerabilities is called the \emph{Boolean Deadlock}, which can appear in a smart contract with improperly implemented semaphores --- parameters that enforce certain order of actions. Funds freeze, in which Ether or tokens cannot be transferred out of the contract, is one of several possible conditions associated with this vulnerability\footnote{Not all freeze conditions indicate a Boolean Deadlock. For example, the Parity Freeze~\cite{browneaccidental} event is not a Boolean Deadlock because it does not involve semaphores.}. Consider the smart contract shown in Fig.~\ref{fig:case3}. This contract allows to deposit money to a virtual ``piggy bank'' and withdraw 80 Shannon\footnote{$1$ Shannon = $10^9$ wei = $1$ Gigawei.} at a time. Another constraint of this contract is that each withdrawal (just like in \textit{Case 1}) must be preceded by one deposit. This logic can operate correctly for a long time. Unfortunately, due to the hidden vulnerability, the user might produce a transaction sequence that will forever lock funds in the contract, as demonstrated in the trace below:
%that follows:
\[
\small
\begin{array}{l}
\text{\ding{182}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{PiggyBank.put}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}} = A_d, \textcolor{Color002}{\textit{msg.value}} = 70000000000\;\text{wei},\\
\;\;\textcolor{Color002}{\textit{this.balance}} = 0,
\textcolor{Color002}{\textit{deposited\_sem}} = false\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textit{this.balance}} = 70000000000\;\text{wei}, \\
\;\;\textcolor{Color002}{\textit{investor}} = A_d, \textcolor{Color002}{\textit{deposited\_sem}} = true \textbf{\rbrack} \\

\text{\ding{183}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{PiggyBank.put}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}} = A_d, \textcolor{Color002}{\textit{msg.value}} = 10000000000\;\text{wei},\\
\;\;\textcolor{Color002}{\textit{this.balance}} = 70000000000,
\textcolor{Color002}{\textit{deposited\_sem}} = true\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textbf{\textit{REVERT}}} \textbf{\rbrack} \\

\text{\ding{184}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{PiggyBank.get}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}}=A_d, \textcolor{Color002}{\textit{investor}}=A_d, \textcolor{Color002}{\textit{deposited\_sem}}=true\\ \;\;\textcolor{Color002}{\textit{this.balance}} = 70000000000\;\text{wei}\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textbf{\textit{REVERT}}} \textbf{\rbrack} \\
\end{array}    
\]
TxT reveals the unexpected behavior of the contract without the knowledge which vulnerability caused the discrepancy between the expected and the actual behavior of the contract. Specifically, before calling the \texttt{put()} function of the \texttt{PiggyBank} smart contract, the user can verify that there is a way to receive money back by submitting a transaction sequence to TxT. If the transaction sequence leads to the deadlock,
%\commentyan{what is Boolean Deadlock?}\commentnick{DONE}
the user will notice  the reversion of a transaction in the wallet, effectively confirming that the sequence is unsafe.

% However, this example poses a very important concern about TxT: the temporal separation of Ethereum transactions. The essence of this problem is that some transaction sequences assume a large time between two or more subsequent transactions, which requires the user to identify and test a sub-sequence of transactions that unambiguously leads to a desirable result for the user. For example, testing only the \texttt{put()} function is insufficient in this contract; instead, the user should test the \texttt{put()}--\texttt{get()} sequence in order to assure the desirable outcome.
%We further discuss the issue of temporal separation of transactions in Section~\ref{}.\commentnick{TODO: resolve ref}

\subsubsection{Case 4: Social Engineering Attacks}

\begin{figure}[t]
    \centering
    \lstinputlisting[language=Solidity]{listings/case4.txt}
    \vspace{-10pt}
    \caption{Case 4: Homograph vulnerability in ERC-20 token.}
    \label{fig:case4}
    \vspace{-10pt}
\end{figure}


Social engineering attacks in smart contracts have gained attention in recent studies~\cite{ivanov2021targeting,torres2019art}. One popular social engineering attack is the Unicode attack~\cite{boucher2021trojan}, also known as the Homograph Attack~\cite{ivanov2021targeting}. Consider the ERC-20 token contract in Fig.~\ref{fig:case4}. This contract allows to buy and sell tokens using Ether cryptocurrency. However, the \texttt{sell()} function has a seemingly innocent verification of the token's currency symbol. %Let us explore why it may cause a problem.

Specifically, the token symbol is set via the token constructor  during the deployment, and it cannot be changed afterwards. This token could be deployed on a testnet (e.g., Rospten) and operate as expected.
%, passing all fathomable unit, manual, or fuzzing tests.
%Let us suppose that 
However, once it is redeployed on Mainnet, one character in the \texttt{pSymbol} parameter of the constructor was replaced with an identically looking character\footnote{For example, the Cyrillic alphabet has a letter that is visually identical to the Latin character ``P'' in most fonts.}. As a result of this replacement, the smart contract will fail to sell the tokens despite the fact that it perfectly worked on a testnet. Moreover, the ERC-20 \texttt{symbol()} function would always return \texttt{SNP}, as expected, but the attempt to sell tokens will nevertheless fail, as shown in the execution trace below (letter `\texttt{P}' in the \texttt{SNP} literal is a Cyrillic letter):
%\commentyan{Again, how TxT can reveal it?}\commentnick{DONE}
%\commentnick{TODO: Fix the buy function trace}
\[
\small
\begin{array}{l}
\text{\ding{182}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{OaklandToken.constructor}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}} = A_d, \textcolor{Color002}{\textit{this.balance}} = 0, \textcolor{Color002}{\textit{initialSupply}} = 0,\\
\;\;\textcolor{Color002}{\textit{pName}} = \text{``Oakland Token''}, \textcolor{Color002}{\textit{pSymbol}} = \text{``SN\textcolor{red}{P}''}
\textbf{)} \\
\;\;\textbf{\lbrack} \textcolor{Color002}{\textit{this.balance}} = 0 \textbf{\rbrack} \\
\text{\ding{183}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{OaklandToken.buy}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.value}}=314159\;\text{wei}, \textcolor{Color002}{\textit{msg.sender}}=A_d, \textcolor{Color002}{\textit{this.balance}} = 0\textbf{)} \\
\;\;\textbf{\lbrack}
\textcolor{Color002}{\textit{this.balance}} = 314159\;\text{wei},
\textcolor{Color002}{\textit{balanceOf}(A_d)} = 314159\;\text{SN\textcolor{red}{P}}
\textbf{\rbrack} \\
\text{\ding{184}}\;\mathrm{\texttt{\textbf{\textcolor{Color001}{OaklandToken.sell}}}} \\
\;\;\textbf{(}\textcolor{Color002}{\textit{msg.sender}}=A_d,
\textcolor{Color002}{\textit{balanceOf}(A_d)} = 314159\;\text{SN\textcolor{red}{P}},\\
\;\;\textcolor{Color002}{\textit{this.balance}} = 314159\textbf{)} \\
\;\;\textbf{\lbrack} 
\textcolor{Color002}{\textbf{\textit{REVERT}}}
\textbf{\rbrack}
\end{array}    
\]
When executing this transaction sequence via TxT, the user will observe the reversion of the \texttt{sell()} transaction in the \texttt{buy}--\texttt{sell} sequence, and thus the user, without auditing the source code, will know that the smart contract is unsafe.
